WikiWhy: Answering and Explaining Cause-and-Effect Questions

As large language models (LLMs) grow larger and more sophisticated, assessing their "reasoning" capabilities in natural language grows more challenging. Recent question answering (QA) benchmarks that attempt to assess reasoning are often limited by a narrow scope of covered situations and subject matters. We introduce WikiWhy, a QA dataset built around a novel auxiliary task: explaining why an answer is true in natural language. WikiWhy contains over 9,000 "why" question-answer-rationale triples, grounded on Wikipedia facts across a diverse set of topics. Each rationale is a set of supporting statements connecting the question to the answer. WikiWhy serves as a benchmark for the reasoning capabilities of LLMs because it demands rigorous explicit rationales for each answer to demonstrate the acquisition of implicit commonsense knowledge, which is unlikely to be easily memorized. GPT-3 baselines achieve only 38.7% human-evaluated correctness in the end-to-end answer & explain condition, leaving significant room for future improvements.

==> tables/emnlp_basic_metrics.tex <==
\begin{table*}[t]
  \centering
    \begin{tabular}{lccccccc}
    \hline\hline
     \textbf{Model} & \multicolumn{7}{c}{\textbf{Fine-tuned GPT-2 vs. Few-shot GPT-3}} \\
     \cmidrule{2-8}
     & S-BLEU & WMD & SMS & BERT-f1 & ROUGE-1 & ROUGE-2 & ROUGE-L \\
    \hline
    \textbf{GPT-2} \\
    ~~~\emph{Greedy}  & 0.042 & 0.541 &
    \textbf{15.81} &
    0.773 & 0.212 & \textbf{0.057} &  0.184 \\
    ~~~\emph{Temp 0.5} & 0.037 & 0.540 &  15.30 & 0.770 &   0.198 &  0.047 &  0.169 \\
    ~~~\emph{Temp 1.0} & 0.022 &  0.536 & 13.25 & 0.760 & 0.161 & 0.022 & 0.134 \\
    \hline
    \textbf{GPT-3}\\
    ~~~\emph{Temp 1.0} & \textbf{0.055} & \textbf{0.555} & 14.93 & \textbf{0.792} & \textbf{0.240} & \textbf{0.057} & \textbf{0.199} \\
    \hline\hline
    \end{tabular}
    \caption{Explanation Evaluation Results of \textbf{CausalQA} dataset according to the following metrics: SacreBLEU (S-BLEU) \citep{post-2018-call}, Word-Mover's distance (WMD) \citep{wmd}, Sentence Mover's Similarity Metrics (SMS) \citep{clark-etal-2019-sentence}, BERT-f1 Score \citep{bert-score}, ROUGE-1, ROUGE-2, and ROUGE-L (all ROUGE-f1 Scores \citep{lin-2004-rouge} averaged). SMS is scaled by 1000 for readability.}
  \label{tab:gpt2v3}
\end{table*}
